MixSup: Mixed-grained Supervision for Label-efficient LiDAR-based 3D Object Detection

Label-efficient LiDAR-based 3D object detection is currently dominated by weakly/semi-supervised methods. Instead of exclusively following one of them, we propose MixSup, a more practical paradigm simultaneously utilizing massive cheap coarse labels and a limited number of accurate labels for Mixed-grained Supervision. We start by observing that point clouds are usually textureless, making it hard to learn semantics. However, point clouds are geometrically rich and scale-invariant to the distances from sensors, making it relatively easy to learn the geometry of objects, such as poses and shapes. Thus, MixSup leverages massive coarse cluster-level labels to learn semantics and a few expensive box-level labels to learn accurate poses and shapes. We redesign the label assignment in mainstream detectors, which allows them seamlessly integrated into MixSup, enabling practicality and universality. We validate its effectiveness in nuScenes, Waymo Open Dataset, and KITTI, employing various detectors. MixSup achieves up to 97.31% of fully supervised performance, using cheap cluster annotations and only 10% box annotations. Furthermore, we propose PointSAM based on the Segment Anything Model for automated coarse labeling, further reducing the annotation burden. The code is available at https://github.com/BraveGroup/PointSAM-for-MixSup.

==> sections/assignment.tex <==
\label{sec:assignment}
For compatibility with the existing 3D detectors, it's necessary to specifically design the assignment strategies for the ground truth clusters.
According to the analysis of ground truth boxes~\citep{survey},
we analogously account for three common situations depending on the assigned object: \textbf{box-based}, \textbf{grid-based}, and \textbf{point-based} assignments.

\paragraph{Box-based}
The box-based approach selects positive samples, i.e., boxes requiring assignment, that exhibit a high intersection over union (IoU) with the ground truth clusters.
The assigned boxes include pre-defined anchors and proposals from detection heads.
As it is impractical to directly calculate the IoU between different representations, we address the challenge by computing the IoU between point clusters within boxes (prediction clusters) and the ground truth clusters.
To align with the notations of ground truth clusters, we denote the prediction clusters as $\hat C=\{\hat s_i\in\{0, 1, 2,\cdots, K\}, \hat g_i\}_{i=1}^N$, where semantic labels $\hat s_i$ 
 and instance IDs $\hat g_i$ of points are consistent with the boxes in which they are placed.
For the points outside the boxes, the semantic labels $\hat s_i$ are set to $0$.
Formally, We define the IoU between the box with ID $m$ and the ground truth cluster with ID $n$ as Eq.~\ref{eq:iou}.
\begin{equation}
\label{eq:iou}
\text{IoU}(m,n)=
\frac{\sum_{i=1}^N\1 (\hat g_i=m)\cdot\1 (g_i=n)}{\sum_{i=1}^N\1 (\hat g_i=m)+\sum_{i=1}^N\1 (g_i=n)-\sum_{i=1}^N\1 (\hat g_i=m)\cdot\1 (g_i=n)}.
\end{equation}
Through Eq.~\ref{eq:iou}, we can assign the ground truth clusters to anchors or proposals and seamlessly support \name to train anchor-based detectors with coarse and accurate labels simultaneously.
\paragraph{Grid-based}
Similar to certain anchor-free methods~\citep{CenterPoint, voxelnext}, the grid-based assignment is suitable for grids, such as voxels, pillars and Bird's Eye View (BEV) feature maps, which assigns the grids near the center of ground truth as positive.
Particularly, we modify the assignment to consider the centers of ground truth clusters.
\paragraph{Point-based}
Some point-based detectors~\citep{pointrcnn, LidarRcnn, FSD} conduct foreground point segmentation for subsequent prediction.
The point-based assignment directly employs ground truth clusters as supervision for detectors, which is equivalent to utilizing ground truth boxes.


==> tables/gtCluster_Kitti_complete.tex <==
\begin{table}[h]
    \small
    \centering
    \caption{Performances on Kitti Dataset}
    \label{tab:gt_kitti_complete}
    % \vspace*{1em}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc}
        \specialrule{1pt}{0pt}{1pt}
        \toprule
        \multirow{2}{*}{Detector} & \multicolumn{3}{c}{\textit{Car} 3D Detection} & \multicolumn{3}{|c|}{\textit{Pedestrian} 3D Detection} & \multicolumn{3}{c}{\textit{Cyclist} 3D Detection}\\
         &  Easy      &   Mod  & Hard &  Easy      &   Mod  & Hard &  Easy      &   Mod  & Hard \\
         \midrule
        % \multicolumn{10}{l}{Fully supervised}\\
        % \midrule
        SECOND (100\% frames)&88.23&78.35&77.05&56.21&52.10&46.89&81.32&67.33&62.50\\
        SECOND (MixSup)&85.40&74.73&67.71&53.36&49.77&45.60&83.83&61.00&57.36\\
        % \midrule
        % \midrule
        % \multicolumn{7}{l}{10\% Sequences Fully supervised}\\
        % \midrule
        % CenterPoint\citep{CenterPoint}&63.58 / 62.98&55.92 / 55.39&65.16 / 56.27&56.97 / 49.07&53.55 / 52.45&51.52 / 50.46\\
        % \midrule
        % \midrule
        % \multicolumn{7}{l}{Weakly supervised: 90\% GT clusters + 10\% GT boxes}\\
        % \midrule
        PV-RCNN (100\% frames)&89.52&83.34&78.73& 65.42&59.27&55.15&86.83&73.25&70.33\\
        PV-RCNN (MixSup)&86.12&76.09&73.89&60.25&54.33&48.87&85.80&65.67&63.09\\
        \bottomrule
        \specialrule{1pt}{1pt}{0pt}
    \end{tabular}
    }
\end{table}

==> tables/gtCluster_Waymo.tex <==
\begin{table}[h]
    \small
    \centering
    \caption{Performances on Waymo Open Dataset validation split.}
    \label{tab:gt_waymo}
    % \vspace*{1em}
    \addtolength{\tabcolsep}{6pt}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|cc|cc|cc}
        \specialrule{1pt}{0pt}{1pt}
        \toprule
        Detector & \multicolumn{2}{c}{\textit{Vehicle} 3D L2 APH} & \multicolumn{2}{|c|}{\textit{Pedestrian} 3D L2 APH} & \multicolumn{2}{c}{\textit{Cyclist} 3D L2 APH}\\
         \midrule
        CenterPoint~\citep{CenterPoint}&65.04&-&61.20&-&67.73&-\\
        FSD~\citep{FSD, FSD_pami}&70.09&-& 69.79&-&73.93&-\\
        % \midrule
        % % \midrule
        % \multicolumn{7}{l}{10\% Sequences Fully supervised}\\
        % \midrule
        % CenterPoint (10\% frames)&63.58 / 62.98&55.92 / 55.39&65.16 / 56.27&56.97 / 49.07&53.55 / 52.45&51.52 / 50.46\\
        \midrule
        CenterPoint (10\% frames)&55.39&-&49.07&-&50.46&-\\
        % \midrule
        % \midrule
        % \multicolumn{7}{l}{Weakly supervised: 90\% GT clusters + 10\% GT boxes}\\
        \midrule
        CenterPoint (\namenospace)&61.83&95.06\%& 57.72&94.31\%&67.46&99.60\%\\
        FSD (\namenospace)&66.08&94.28\%&66.53& 95.33\%&73.09&98.86\%\\
        \bottomrule
        \specialrule{1pt}{1pt}{0pt}
    \end{tabular}
    }
    \addtolength{\tabcolsep}{-6pt}
\end{table}

==> tables/gtCluster_Waymo_complete.tex <==
\begin{table}[h]
    \small
    \centering
    \caption{Performances on Waymo Open Dataset}
    \label{tab:gt_waymo_complete}
    % \vspace*{1em}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|c|c|c|c|c|c}
        \specialrule{1pt}{0pt}{1pt}
        \toprule
        \multirow{2}{*}{Detector} & \multicolumn{2}{c}{\textit{Vehicle} 3D AP/APH} & \multicolumn{2}{|c|}{\textit{Pedestrian} 3D AP/APH} & \multicolumn{2}{c}{\textit{Cyclist} 3D AP/APH}\\
         &  L1      &   L2     &   L1      &   L2  &   L1     &   L2\\
         \midrule
        % \multicolumn{7}{l}{Fully supervised}\\
        % \midrule
        CenterPoint (100\% frames)&73.54 / 73.00&65.53 / 65.04&74.91 / 68.44&67.16 / 61.20&71.51 / 70.34&68.85 / 67.73\\
        % FSD\citep{FSD}&79.20 / 78.76&70.49 / 70.09&83.22 / 78.02&74.62 / 69.79&77.76 / 76.62&75.04 / 73.93\\
        % \midrule
        % \midrule
        % \multicolumn{7}{l}{10\% Sequences Fully supervised}\\
        % \midrule
        CenterPoint (10\% frames)&63.58 / 62.98&55.92 / 55.39&65.16 / 56.27&56.97 / 49.07&53.55 / 52.45&51.52 / 50.46\\
        % \midrule
        % \midrule
        % \multicolumn{7}{l}{Weakly supervised: 90\% GT clusters + 10\% GT boxes}\\
        % \midrule
        CenterPoint (MixSup)&70.36 / 69.81&62.32 / 61.83&71.77 / 64.92&63.96 / 57.72&71.12 / 70.02&68.53 / 67.46\\
        % FSD&75.28 / 74.74&66.57 / 66.08&80.58 / 74.86&71.79 / 66.53&76.87 / 75.77&74.16 / 73.09\\
        \bottomrule
        \specialrule{1pt}{1pt}{0pt}
    \end{tabular}
    }
\end{table}

==> tables/gtCluster_nuScenes.tex <==
\begin{table}[h]
    \small
    \centering
    \caption{Performances on nuScenes validation split.}
    \label{tab:gt_nuscenes}
    % \vspace*{1em}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|cc|cc|cccccccccc}
        \specialrule{1pt}{0pt}{1pt}
        \toprule
        Detector & \multicolumn{2}{|c|}{mAP}   &  \multicolumn{2}{|c|}{NDS}  & Car  & Truck & C.V.  & Bus   & Trailer & Bar.  & Mot. & Byc. & Ped. & T.C.   \\
        % \midrule
        % \midrule
        % \multicolumn{13}{l}{Fully supervised}\\
        \midrule
        CenterPoint&62.41&- & 68.20 &- & 84.94 & 57.92 & 22.78 & 71.64 & 37.12 & 67.46 & 68.23 & 57.68 & 85.29 & 71.07\\
        % \midrule
        % \midrule
        % \multicolumn{13}{l}{10\% Sequences Fully supervised}\\
        \midrule
        CenterPoint (10\% frames)&42.19 & - & 55.38 & - & 77.18 & 38.18 & 3.60 & 42.17 & 9.12 & 59.29 & 36.31 & 20.54 & 78.97 & 56.57\\
        % \midrule
        % \midrule
        % \multicolumn{13}{l}{10\% GT boxes}\\
        % \midrule
        % CenterPoint&9.30 & 39.89& 64.12 & 5.02 & 0.00 & 5.19 & 0.00 & 7.55 & 3.28 & 3.88 & 3.66 & 0.25\\
        % \midrule
        % \midrule
        % \multicolumn{13}{l}{Weakly supervised: 90\% GT clusters + 10\% GT boxes}\\
        \midrule
        CenterPoint (MixSup) &60.73 &97.31\% & 66.46 &97.45\%  & 83.37 & 55.29 & 20.25 & 69.19 & 37.87 & 67.52 & 65.93 & 54.08 & 84.51 & 69.27\\
        % \midrule
        % \midrule
        % \multicolumn{13}{l}{Weakly supervised: Generated clusters + 10\% GT boxes}\\
        % \midrule
        % CenterPoint&48.04 & 58.93& 73.41 & 44.93 & 12.44 & 63.40 & 21.28 & 33.81 & 58.66 & 45.01 & 79.63 & 47.85\\
        \bottomrule
        \specialrule{1pt}{1pt}{0pt}
    \end{tabular}
    }
\end{table}

==> tables/gtCluster_nuScenes_complete.tex <==
\begin{table}[h]
    \small
    \centering
    \caption{Performances on nuScenes}
    \label{tab:gt_nuscenes_complete}
    % \vspace*{1em}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|cc|cccccccccc}
        \specialrule{1pt}{0pt}{1pt}
        \toprule
        Detector & mAP   &    NDS  & Car  & Truck & C.V.  & Bus   & Trailer & Bar.  & Mot. & Byc. & Ped. & T.C.   \\
        \midrule
        % \midrule
        % \multicolumn{13}{l}{Fully supervised}\\
        % \midrule
        CenterPoint (100\% frames)&62.41 & 68.20 & 84.94 & 57.92 & 22.78 & 71.64 & 37.12 & 67.46 & 68.23 & 57.68 & 85.29 & 71.07\\
        % \midrule
        % \midrule
        % \multicolumn{13}{l}{10\% Sequences Fully supervised}\\
        % \midrule
        CenterPoint (10\% frames)&42.19 & 55.38& 77.18 & 38.18 & 3.60 & 42.17 & 9.12 & 59.29 & 36.31 & 20.54 & 78.97 & 56.57\\
        % \midrule
        % \midrule
        % \multicolumn{13}{l}{10\% GT boxes}\\
        % \midrule
        % CenterPoint&9.30 & 39.89& 64.12 & 5.02 & 0.00 & 5.19 & 0.00 & 7.55 & 3.28 & 3.88 & 3.66 & 0.25\\
        % \midrule
        % \midrule
        % \multicolumn{13}{l}{Weakly supervised: 90\% GT clusters + 10\% GT boxes}\\
        % \midrule
        CenterPoint (MixSup)&60.73 & 66.46 & 83.37 & 55.29 & 20.25 & 69.19 & 37.87 & 67.52 & 65.93 & 54.08 & 84.51 & 69.27\\
        % \midrule
        % \midrule
        % \multicolumn{13}{l}{Weakly supervised: Generated clusters + 10\% GT boxes}\\
        % \midrule
        % CenterPoint&48.04 & 58.93& 73.41 & 44.93 & 12.44 & 63.40 & 21.28 & 33.81 & 58.66 & 45.01 & 79.63 & 47.85\\
        % \midrule
        % \midrule
        % \multicolumn{13}{l}{Weakly supervised: Generated clusters (Filter FP) + 10\% GT boxes}\\
        % \midrule
        % CenterPoint\citep{CenterPoint}&50.91 & 60.51& 74.46 & 48.28 & 16.23 & 62.23 & 26.32 & 57.39 & 53.23 & 40.51 & 78.53 & 51.94\\
        \bottomrule
        \specialrule{1pt}{1pt}{0pt}
    \end{tabular}
    }
\end{table}

==> tables/implementation.tex <==
\begin{table}[h]
    \centering
    % \vspace{-8pt}
    \caption{Detailed implementation on of four detectors on three datasets.}
    \label{tab:implementation}
    % \vspace*{1em}
    % \addtolength{\tabcolsep}{6pt}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|cccc}
        \specialrule{1pt}{0pt}{1pt}
        \toprule
        Detector &Batch Size (per GPU)& Schedule (epochs) & Learning Rate & Fadeing Epochs\\
         \midrule
        \rowcolor{semi_color}SECOND&4&80&0.003&-\\
        \rowcolor{semi_color}PVRCNN&2&80&0.01&-\\
        \rowcolor{self_color}CenterPoint&4&30&0.003&5\\
        \rowcolor{self_color}SECOND&4&30&0.003&-\\
        \rowcolor{self_color}PV-RCNN&2&30&0.01&5\\
        \bottomrule
        \specialrule{1pt}{1pt}{0pt}
    \end{tabular}
    }
    % \addtolength{\tabcolsep}{-6pt}
    \vspace{-10pt}
\end{table}
